Question Relatedness on Stack Overflow: The Task, Dataset, and Corpus-inspired Models

Domain-specific community question answering is becoming an integral part of professions. Finding related questions and answers in these communities can significantly improve the effectiveness and efficiency of information seeking. Stack Overflow is one of the most popular communities that is being used by millions of programmers. In this paper, we analyze the problem of predicting knowledge unit (question thread) relatedness in Stack Overflow. In particular, we formulate the question relatedness task as a multi-class classification problem with four degrees of relatedness. We present a large-scale dataset with more than 300K pairs. To the best of our knowledge, this dataset is the largest domain-specific dataset for Question-Question relatedness. We present the steps that we took to collect, clean, process, and assure the quality of the dataset. The proposed dataset Stack Overflow is a useful resource to develop novel solutions, specifically data-hungry neural network models, for the prediction of relatedness in technical community question-answering forums. We adopt a neural network architecture and a traditional model for this task that effectively utilize information from different parts of knowledge units to compute the relatedness between them. These models can be used to benchmark novel models, as they perform well in our task and in a closely similar task.

==> dumpster.tex <==
%%%%%%%%%%%%%%%%%  FROM INTRO


\begin{comment}
o find related \ku{}s solutions and perspective to similar problems. 
Therefore, \emph{identification of related \ku{}s} can be very helpful in efficient guiding exploration of knowledge.


becomes very important. Identification of related \ku{}s helps developers to retrieve target knowledge more efficiently\FFix{Amin: ??}. 

\Fix{Amin: should we remove the following sentence? David: I agree.}
Developers can use relevant \ku{}s to better understand the proposed solutions and the implications of each proposal, and sometimes to better understand the programming problem at hand.


In addition to fiding the most relavent post to the questions, askers often wishes to be able to find other relavent information to better understand the solutions presnted on each posts, and sometimes understand the the problem better.
Therefore, it is desirable to find \emph{relevant} information to the current posts to explore information regarding to variants of the problem, such as different systems, assumptions, or information about the ingeridiants of the current solutions.

various information needs for developing programs. 
\Fix{A sentence here :)}
They usually use online forums and weblogs to satisfy these needs. 
One of the main locations to look for information is \SO{}. Streack Overflow is the largest online community for developers to learn and share their programming knowledge.\footnote{https://stackoverflow.com/}

Nowadays, \SO{} is an indispensable tool in developers' professional life.
They can use \SO{} to find answers to their questions, or to post their questions.
Crowd in \SO{} is very efficient. 
Most questions are being answered in minutes after posting the question, which has made \SO{} the most popular question answering website for developers~\cite{Mamykina:2011:CHI}.

TODO

In many developer online forums like Stack Overflow, computer programming knowledge has been shared through millions of questions
and answers. 

In most of these forums, a user asks a question and recieve a variety of answers from other users. 
The question and answers in one thread are likely to be related to information provided in
other threads. 


When asking a question or providing an answer in Stack Overflow, users reference existing questions and answers that contain relevant knowledge by URL sharing~\cite{xu2016predicting}.
The fundamental goal of finding and ultimately closing duplicate questions is to help people find the right answer by getting all of those answers in one place~\cite{StackOverflowduplicate}.

However, it takes efforts for users to go through different post and annotate related posts, and users can benefit from automated tools to 






Question-question similarity in cQA field is considered as an important problem with application
to question recommendation, question duplicate
detection, community question answering,
and question answering in general~\cite{nakov2017semeval}.

Existing datasets typically focus on binary relatedness (i.e., duplicate or not) ...

In this paper, we set out the task of collecting a standard corpus of question pairs from \SO with different levels of similarity. We formulate the problem of question-question similarity as a multi-class
classification problem. More precisely, given two questions, 
the cQA system has to infer the degree of relevancy of the two questions by choosing one relatedness (relevancy) class.


% Why is it interesting and important?

When users search or explore different questions in a forum, having more information about the relevancy of posts can support users' targeted information needs.

% Why is it hard? (E.g., why do naive approaches fail?)
When dealing with real-world data, presence of informal, redundant, unrelated text and in our case, technical jargons constitutes a major challenge in prediction of similarity level between two posts. 

% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)



% What are the key components of my approach and results? Also include any specific limitations.

To asses the level of difficulty of our dataset, 



While other studies exclude code parts for learning the similarity of the two question[][], we decided to use this part as an other informative source. 
We believe code snippets are the most important part of questions and answers and the the text can be seen as a complementary part to explain the code. 

Many studies have been done on code clone detection[][] and also natural aspect of code[], however, we decided to extract information as much as possible by just looking at at the code as natural text. We provide more information in section [method]
%%%%%%%%%%%%%%%%%%%%%%%%%%%Important:
% We believe the type of similarity between two \ku{} can have relationship more than only duplicate and non-duplicate
These types of relationships are important to users in developing forums because usually they are novice and don't know the actual terminology for their problem, so providing related questions can help them find the solution.   

\SO is an indispensable part of developers' professional life. 
I


Comparing Stack overflow to other community question answering
websites like Yahoo answers or Qatar living, we can observe that
there are more technical terms in stack overflow which makes this forum so
special. 

Identifying relevant posts is not considered as an easy task. There
might be many cases in which the two given questions
share few common words, but they embody
strongly relevant knowledge. To overcome the lexical gap, we propose a model with the ability to identify semantic relations between questions. Our model employs
deep learning techniques to detect the relevancy
of questions in the Stack overflow. The model is able to capture the similarity of domain-specific
concepts in questions. Moreover, we enhance the proposed model by using hand-crafted features. 



\end{comment}


==> experiment.tex <==
% \section{Results and Discussion}

% % \Fix{David: My 2 cents is, maybe this section can be renamed: Experiment Results :-) ? Preprocessing may be moved either to the dataset/experiment setting section and part of the implementation moved to the experiment setting section too :-) Maybe this section can focus more on the results and a description on what it means :-) ? Just my 2 cents :-) Please feel free to ignore -- I have never written a COLING paper :-) Reza: DOne}
% % In this section, we assess the effectiveness of hand-crafted features. 
% % Then, we report the performance of  baseline SVM model and Dot\_BiLSTM model. 
% % Finally, we provide an analysis of the results.

% % Part{Individual features on \kua{}'s text }
% % In order to assess the contribution of individual features to the classification, we build and evaluate an SVM model for each feature separately. As shown in Figure~\ref{fig:featureText}, the results indicate that
% % Soft-cosine features slightly outperform other features in natural text part of \ku{}s.


% % \begin{figure}[htbp]
% % \centering
% %   \includegraphics[width=0.7\textwidth]{figs/featureText}
% %   \caption{\small Results of the model by considering different features. Text selection: title, body and answers. Soft\_cos\_google\_W2V: soft-cosine similarity with Google news W2v, Soft\_cos\_SO\_W2V: soft-cosine similarity with \SO{} W2V and Soft\_cos\_LEV: soft cosine similarity with Levenshtein distance}
% %   \label{fig:featureText}
% % \end{figure}

% % \noindent \textbf{Individual features on \kua{}'s code: }
% % We extract similar features for code snippets to find important features in those sections. 
% % % Note that for computing Soft\_cos\_SO\_W2V, we use our word2vec model trained on code parts of the \SO{} dataset (explained in section~\ref{section:features}). 
% % Figure~\ref{fig:featureCode} depicts the performance of each feature in the prediction of relatedness of \ku{}s. 
% % Models based on \softSO{} and \softLev{} features perform better on code parts. 
% % By comparing the results between Figure~\ref{fig:featureText} and Figure~\ref{fig:featureCode}, we find that text parts is been more effective in predicting relatedness of \ku{}s. 
% %Comparing results of text and code, text has better performance over all features\Fix{Amin: why do we compare the code with text? Is there any insight here? Reza: No, I thought it might be interesting, do I need to remove it? }.
% %Results of the model by considering different features. Text selection: bodyCode + answerCode
% % \begin{figure}[htbp]
% %     \centering
% %     \begin{minipage}{0.45\textwidth}
% %         \centering
% %         \includegraphics[width=1\textwidth]{figs/featureText2.png}
% %         \caption{\small Results of the model by considering different features. Text selection: title, body and answers.
% %         % \Space{ Soft\_cos\_google\_W2V: soft-cosine similarity with Google news W2v, Soft\_cos\_SO\_W2V: soft-cosine similarity with \SO{} W2V and Soft\_cos\_LEV: soft cosine similarity with Levenshtein distance}
% %         }
% %   \label{fig:featureText}
% %     \end{minipage}\hfill
% %     \begin{minipage}{0.45\textwidth}
% %         \centering
% %         \includegraphics[width=1\textwidth]{figs/featureCode2.png}
% %         \vspace{-0.5cm}
% %         \caption{\small Results of the model by considering different features. Text selection: bodyCode + answerCode.
% %         % \Space{Soft\_cos\_google\_W2V: soft-cosine similarity with Google news W2v, Soft\_cos\_SO\_W2V: soft-cosine similarity with \SO{} W2V and Soft\_cos\_LEV: soft cosine similarity with Levenshtein distance}
% %         }
% %   \label{fig:featureCode}
% %     \end{minipage}
% % \end{figure}
% % \begin{figure}[htbp]
% % \centering
% %   \includegraphics[width=0.7\textwidth]{figs/featureCode.png}
% %   \caption{\small Results of the model by considering different features. Text selection: bodyCode + answerCode. Soft\_cos\_google\_W2V: soft-cosine similarity with Google news W2v, Soft\_cos\_SO\_W2V: soft-cosine similarity with \SO{} W2V and Soft\_cos\_LEV: soft cosine similarity with Levenshtein distance}
% %   \label{fig:featureCode}
% % \end{figure}

% % \Part{Combination of the best features from textual and code parts }
% % Table~\ref{table:textSelection} depicts the performance of models that use the combination of the best performing features: cosine similarity, \softSO{}, \softgoog{}, and \softLev{}, on the different part of data selection.
% % Among individual parts (Models 1--4), body and answers (Model 1 and 2) perform slightly better than other parts.
% % % Model 5 that includes all parts of \ku{}s except code snippets performs better than individual parts.
% % We consider model 6 as our baseline, that includes all parts as well as code, and achieve the highest performance. 
% % Taking into account the code parts in our experiments, improves our results by two percent. 
% % \begin{table}[htbp]
% % \small
% % \centering
% % \caption{\small 
% % Results of different text selections. Features for text parts: Cosine similarity, \softSO{}, \softgoog{}, and \softLev{}. Features for code parts: \softSO{}, \softLev{}}
% % \label{table:textSelection}
% %  \resizebox{\columnwidth}{!}{
% % \begin{tabular}{|l|l|l|l|l|l|}
% % \hline
% % Models&	Text selection/metrics      & F-micro & Precision & Recall \\ \hline
% % Model 1&	Title                                &       0.47         &     0.44      &   0.48     \\ \hline
% % Model 2&	Body                               &     0.51           &    0.49       &   0.51     \\ \hline
% % Model 3&	Answers                            &      0.51          &   0.5        &      0.51  \\ \hline
% % Model 4&	Codes                                 &     0.4           &     0.42      &   0.4     \\ \hline
% % Model 5&	Title, Body, Answers                       &      0.59          &     0.58      &   0.59     \\ \hline
% % Model 6&	Title, Body, Answers, Codes           &    0.61            &     0.6      &   0.61     \\ \hline
% % \end{tabular}
% % }
% % \end{table}


% % \Part{Dot\_BiLSTM results}
% \Part{Analysis of Results }
% Our experimental results in Table~\ref{tab_results} show the effectiveness of our Dot\_BiLSTM model. 
% % Table \ref{tab_results} shows the baseline and Dot\_BiLSTM's results. 
% Comparing these two models, we realize that Dot\_BiLSTM substantially outperforms baseline by more than 12\% f-score and 14\% and 13\% precision and recall, respectively. This demonstrates that our deep learning model can predict the relatedness between \ku{}s more effectively. 
% %The significant improvement obtained by the proposed model indicates the superiority of neural network over traditional models for this specific task.  
% % \Part{The difficulty of predicting individual classes} 
% Tables~\ref{table:classes} shows f-scores for predicting for individual classes.
% It shows that the Isolated class is relatively easier to distinguish by both models compared to other classes.
% Comparing results of the individual classes, Dot\_BiLSTM, in predicting the Isolated, Duplicate and Indirect classes performs better than the baseline model. 
% For the Direct class, both models perform similarly.

% \begin{table}[]
% \centering
% \caption{Results for the traditional and the neural models}
% \label{tab_results}
% \begin{tabular}{|l|l|l|l|}
% \hline
% Model/Metrics  & F-score & Precision & Recall \\ \hline
% Traditional       & 0.59           & 0.58      & 0.59   \\ \hline
% Dot\_BiLSTM & 0.73            & 0.74       & 0.74   \\ \hline
% \end{tabular}
% \end{table}



% %: Considering the best-performing features: Cosine similarity, \softgoog{}, \softSO{} and \softLev{} in title, body, and answers parts as well as \softSO{} and \softLev{} in code parts

% \begin{table}[htbp]
% \centering 
% \caption{\small Comparing the results (f-score) of Baseline (model 6) and Dot\_BiLSTM models.}
% \label{table:classes}
% \resizebox{\columnwidth}{!}{%  
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% Classes     & Duplicate & Direct &       Indirect &         Isolated & Overall: Micro \\ \hline
% Traditional    & 0.53      & 0.57        & 0.44          & 0.79     & 0.59           \\ \hline
% Dot\_BiLSTM & 0.84         & 0.57        & 0.63          & 0.90     & 0.74           \\ \hline
% \end{tabular}
% }
% \end{table}


% \Part{Reformulating the problem to the binary Duplicate Question Detection}

% \FFix{managing data}

% \FFix{results for DQD}

% \Part{The performance of the models on other dataset}\label{sec:askubuntu}

% \FFix{adding results for ASKUbuntu}

% \FFix{Comparing the charactersitics and results between our DS and AskUbuntu}

% \Part{The Importance of Code Parts } 
% The results of the baseline experiments show that the code component in \ku{}s can improve the performance of classifiers.
% The modest increase in performance (only $2\%$) of classifiers by using raw source code can suggest that with the extraction of more sophisticated features from code snippets, we may be able to achieve higher performance in both traditional and deep learning models. 
% %The deep learning neural model performed better than the SVM.

% \Part{More To Explore }

% \FFix{adding code}

% In our experiments, we purposely confine our models to only utilize information in \emph{Title}, \emph{Body}, \emph{Answers} and \emph{Code parts}. However, relying on other parts of dataset like \emph{BestAnswer} and \emph{Tags} can open new gates for this task.


% % \Comment{
% % \subsection{Neural network models}


% % \begin{table}[]
% % \centering
% % \caption{F1-scores for neural network models}
% % \label{my-label}
% % \begin{tabular}{|l|l|l|l|l|l|}
% % \hline
% % Model/Class                & Duplicate & Direct & Indirect & Isolated & Overall \\ \hline
% % Model1 Aggregation Network        & 0.72      & 0.61   & 0.73     & 0.85     & 0.73    \\ \hline
% % Model2 Siamese Network            & 0.72      & 0.60   & 0.64     & 0.81     & 0.69    \\ \hline
% % \end{tabular}
% % \end{table}
% % }



% % \Comment{
% % Since the code and also text parts contain technical words, specific preprocessing is needed to convert them to the normal form:
% % }


% % \Comment{
% % More representations of code representations, such as graphs~\cite{allamanis2018learning} or semantic embeddings~\cite{func2vec} can be explored to improve the accuracy of models.
% % }

% % \Comment{
% % We believe that splitting concatenated words can convert words to a standard form on both sides which is useful for capturing similarity based on introduced features. 
% % \Fix{Amin: a stronger argument please}. 
% % Other preprocessing steps on the text and code\Fix{Amin: is there anything other than text and code? If not why not say `\ku{}'.Reza: we can say ku but each ku has different texts and codes } include: lowercasing the words, replacing URLs and numbers with the generic terms, and removing punctuation marks.
% % We only remove stop-words from text because removing stop-words from code would results in information loss in like words $this$ in programing languages.
% % }



% % \Comment{
% % Table 2 shows the results of our model with different configurations. This table gives f1-scores for each class separately and it also provides the overall micro f1-score. In the first and the second configurations, we only have one of the CNN or BiLSTM models for getting questions representations. As it is shown in the first and the second models, BiLSTM alone performed better than CNN. (All other layers and configurations remained unchanged). However, by combining both representations, we can get better results (model 9), this suggests that these two representations can complement each other and together can give a better representation of the input.

% % Instead of concatenation, we first try dot product to get cosine similarity of two representations. The results for concatenation was better than cosine similarity by two percent.

% % As we explained in the method section, adding the representation of the first question after the first dense layer, improves the results. Model 4, 5, 6 and 9 show different configurations when we add question 1, question 2, both of them and none of them to the model. As we see, model 3 without adding any question performs near 3 percent less than when we add question 1 to the model. When we add both questions or only question 2, the results is near when we add question 1 only. Since the model is symmetry, adding question 1 or 2 should not be different. The small difference can be explained by the variation between first and second question in the data set. In our experiment, adding only question 1 gives us the best result.

% % Using hand-crafted features boosts our results significantly. In our experiment, we first used each traditional features separately to see the contribution of each feature. All of them have a positive impact on results between 0.4-0.8. Then we added features one by one to the model. As a result, these features boost our results by three percent. The third model shows lower f-score when we don't consider hand-crafted features in our model. We choose these features because of their good performance in previous studies. Perhaps having more features can result in a better model. We will investigate the impact of more features in our future works. 

% % We tried two different sources of word embedding. The first one is Glove [3] which is a general word embedding and the second one is Stack overflow (SO) pre-trained word2vev [2]. This embedding (SO) is trained on 100,000 unannotated questions and their answers from Stack overflow forum. The number of null word embedding (out of vocabulary) for Glove is 8508 and for Stack overflow word2vec is 5256. This shows pre-trained word embedding on Stack overflow has less out of vocabulary words in compared to Glove. As it is shown in model 7 in Table 2, the proposed model performs similarly when we use Glove word embedding or Stack overflow word embedding.

% % In preprocessing subsection, we explained how we apply special preprocessing on technical words. Model 7 in Table 2 indicates that without having technical preprocessing, we get lower performance. This emphasizes the importance of suitable preprocessing on data.

% % \begin{table*}[]
% % \footnotesize
% % \centering
% % \caption{Different configurations for proposed model}
% % \label{my-label}
% % \begin{tabular}{|l|l|l|l|l|l|l|}
% % \hline
% %   & Model/Class                                 & Duplicate & Direct Link & Indirect Link & Isolated & Overall \\ \hline
% % 1 & BiLSTM                                      & 0.965     & 0.959       & 0.99          & 0.97     & 0.947   \\ \hline
% % 2 & CNN                                         & 0.95      & 0.95        & 0.98          & 0.96     & 0.92    \\ \hline
% % 3 & CNN\_BiLSTM without hand-crafted features   & 0.956     & 0.94        & 0.99          & 0.95     & 0.924   \\ \hline
% % 4 & CNN\_BiLSTM without adding any question     & 0.91      & 0.86        & 0.97          & 0.94     & 0.852   \\ \hline
% % 5 & CNN\_BiLSTM by adding both q1 and q2        & 0.96      & 0.95        & 0.99          & 0.98     & 0.947   \\ \hline
% % 6 & CNN\_BiLSTM by only adding q2               & 0.96      & 0.95        & 0.988         & 0.983    & 0.942   \\ \hline
% % 7 & CNN\_BiLSTM without technical preprocessing & 0.96      & 0.956       & 0.99          & 0.98     & 0.94    \\ \hline
% % 8 & CNN\_BiLSTM by using GLOVE word embedding   & 0.968     & 0.957       & 0.993         & 0.985    & 0.952   \\ \hline
% % 9 & (Proposed model) CNN\_BiLSTM                & 0.966     & 0.96        & 0.995         & 0.98     & 0.952   \\ \hline
% % \end{tabular}
% % \end{table*}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%
% % By comparing achieved results for each class, we can observe that indirect link is the easiest class to predict for most cases. On the other hand, direct link is the hardest class to predict. We compared the predicted results for each class and realized that direct link and duplicate class are similar to each other and have the most misclassified examples with each other.
% % %%%%%%%%%%%%%%%%%%%%%%%%%%
% % For configuration part, we set to consider only maximum 60 first words of each text as input. We tried different sizes, but considering the first 60 words in our data performed the best among tested values 20, 40 and 50. After having more accurate observation on data, we understood that in most cases the size of topic following by first lines of body is not more than 60 words. So 60 words as input can provide enough information.
% % We applied padding at the end of small sentences to have the same size for all inputs. We trained our models for 25 epochs. We used categorical cross-entropy as a loss function and Adam for optimization. In training phase, we saved model weights from the model check point with the maximum validation accuracy.  
% % %%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure}[h!]
% % \centering
% %   \includegraphics[width=0.6\textwidth]{figs/chart.png}
% %   \caption{Comparing proposed model with previous works on the same data set.}
% %   \label{F1-score}
% % \end{figure}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%

% % Figure 5 compares the results (micro f1-score) of our model to other two previous works by Xu et al. [1] and Wei et al. [2] on the same data set. As it is shown, the proposed model outperformed other works for all classes. 
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \subsection{Qualitative Analysis}
% % Tables 3-6 present some examples of each class and correct predicted class. Table 3 shows an example of a duplicate questions pair. In this example, two question don't have many words in common. However, the proposed model could correctly identify the correct semantic similarity between two questions. In the second example (Table 4), we have a directly linked pair of questions. Both questions have few words in common. However, some phrases like \texttt{text not displaying correctly} and \texttt{GUI repaint() problem} can be considered as directly linked concepts. Simple word matching techniques would not be able to capture such semantic similarities. Our model correctly labeled them as direct link. Table 5 shows an example of two questions with indirect link relation. Our system was able to identify the small relation between the questions correctly. 
% % Table 4 contains an example of two isolated questions. Although these questions share several words with each other, they are not related to each other. Our system can correctly detect the low level (no) similarity.
% % \subsection{Error Analysis}
% % In the last section, we talked about how our model was able to correctly predict semantic relationships without relying on the number of common words. In this section, we investigate cases which our model was unable to predict correctly. As we mentioned earlier, most of the misclassifications are for duplicate class and direct link class.
% % Table 7 gives the one example of this case. The correct label shows two questions are duplicate however our model predicted direct link class. The first question is asking for a way to handle large numbers in java. In two of its answers, conversion to binary is suggested. The second example, is asking about conversion large numbers to binary. these two questions are not exactly similar to each other but in comments of first one the second question is suggested. So direct link also seems as a reasonable choice. However, since the binary conversion is suggested at the very end of the first thread, our model is not able to capture that. We only consider the first 60 words as input for each question. If comments we given separately in the data set, we could have separate representation for them. We will consider this as our next step in our future works.
% % }

